The Expressive Power of Tuning Only the Normalization Layers

Feature normalization transforms such as Batch and Layer-Normalization have become indispensable ingredients of state-of-the-art deep neural networks. Recent studies on fine-tuning large pretrained models indicate that just tuning the parameters of these affine transforms can achieve high accuracy for downstream tasks. These findings open the questions about the expressive power of tuning the normalization layers of frozen networks. In this work, we take the first step towards this question and show that for random ReLU networks, fine-tuning only its normalization layers can reconstruct any target network that is $O(\sqrt{\text{width}})$ times smaller. We show that this holds even for randomly sparsified networks, under sufficient overparameterization, in agreement with prior empirical work.

==> App_numerical.tex <==

\begin{figure}[h!]
    \centering
    \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=0.49\textwidth]{Neurips/figures/Training_synth_sparsity_1.0.pdf}
        \hfill
         \includegraphics[width=0.49\textwidth]{Neurips/figures/Training_synth_input_dim_25_sparsity_1.0.pdf}
     \end{subfigure}
     
    \caption{Verifying our constructions for \acl{BNshort} parameters on data created by a random neural network $g$. The baseline algorithm (Blue curve) corresponds training the \acl{BNshort} parameters of the network $f_1$ on this data using SGD, while the other parameters (weight matrices) are kept frozen at initialization. The green curve represents the network $f_2$ created by our construction by directly using the teacher network $g$. We also train a dense neural network $g'$ with same architecture as $g$ using SGD (dashed black curve). We then use our construction on $g'$ to create $f_3$, which is represented by the orange curve. In the figure on the left, we vary the width of the hidden layer of $g$, and set the width of $f_1,f_2,$ and $f_3$ to be the one proposed in Theorem \ref{th: width}. In the figure on the right, we fix the width of $g$ to be 25, and vary the widths of $f_1,f_2,$ and $f_3$. }
        


    \label{fig:exp1}
\end{figure}
To verify our construction numerically, we designed the following experiment: We create a random target network $g(\vx)$ with one hidden layer of width $d$, with ReLU activations. The output of the target network is simply the sum of outputs of the hidden layer neurons. We try to learn this function using the network $f(\vx)$ from Theorem \ref{th: width} using three algorithms
\begin{itemize}
    \item Baseline: We freeze the weight parameters of $f$ and train only the \acl{BNshort} parameters using SGD.
    \item Constructive algorithm, directly from target network: We freeze the weight parameters of $f$ and set the \acl{BNshort} parameters according to the construction prescribed in the proof of Theorem \ref{th: width}.
    \item Constructive algorithm, from a dense learnt network: For this approach, we first take another random network $g'$ with the same architecture as $g$, and train it using SGD on the data generated by $g$. Then, we create $f$ by freezing its weight parameters and setting the \acl{BNshort} parameters according to the construction prescribed in the proof of Theorem \ref{th: width}, but using $g'$ in the construction instead of $g$. 
\end{itemize}
The results are shown in Figure \ref{fig:exp1} (left). We see that both the constructive algorithms beat the baseline. These show that training \acl{BNshort} parameters using SGD might not be the best algorithm. While the constructive algorithm which uses the target network directly might be impossible to use in practice, the constructive algorithm that first trains a dense network and uses that to construct the \acl{BNshort} parameters shows that there can be other, indirect ways of training \acl{BNshort} parameters, which are better than simply using SGD. 

To see the dependence of error on the width of $f$ for the three algorithms, we fixed the width of $g$ to be $d=25$, and repeated the first experiment with varying widths of $f$. The results for this experiment are shown in Figure \ref{fig:exp1} (right). Here we see that while at smaller widths the baseline (SGD) performs better (still only achieves a constant loss), as the width increases, our constructive algorithms beat SGD.
Note that here we used pseudo-inverse for setting the \acl{BNshort} parameters of $f$ using our construction, since at lower widths, the matrices that need to be inverted become rank-deficient. 

We present the results of some additional experiments along with the details of the experiment in the next section.


